Decoupled Context Processing for Context Augmented Language Modeling

Language models can be augmented with a context retriever to incorporate knowledge from large external databases. By leveraging retrieved context, the neural network does not have to memorize the massive amount of world knowledge within its internal parameters, leading to better parameter efficiency, interpretability and modularity. In this paper we examined a simple yet effective architecture for incorporating external context into language models based on decoupled Encoder Decoder architecture. We showed that such a simple architecture achieves competitive results on auto-regressive language modeling and open domain question answering tasks. We also analyzed the behavior of the proposed model which performs grounded context transfer. Finally we discussed the computational implications of such retrieval augmented models.

==> context.tex <==
\newcommand\todo[1]{\textcolor{red}{TODO: #1}}

\subsection{Context and Language Modeling Scores} \label{sec:long-short} 

For language modeling, we looked at how the extra context can affect the probability of each target token. To do the analysis, we used two language models of same size trained in the language modeling experiment in Section~\ref{sec:lm-experiment}. One is trained with retrieved context and one is trained without context. Then we inference both models on the C4 validation split and collect the log likelihood of the target tokens. We used NLTK~\cite{bird2009natural} to assign each target token a Part of Speech tag. Note that NLTK tokenizes the sentence slightly different from ours, which is sentencepiece. To bridge the gap, we mapped the boundary of both NLTK tokens and sentence piece tokens to unicode code unit. If the sentence piece token contains multiple NLTK tokens, the tagging is based on majority vote. If the sentence piece token is part of a NLTK token, it's assigned that NLTK token's tag. We further looked at whether the target token has appeared in the retrieved context and the input sequence. We measured the percentage of improvement on log likelihood on the target tokens when there's context. The results are in Figure~\ref{fig:in_long_in_short}. There are two observations:

First, different types of tokens benefit differently from the context. Noun (NN, NNP, NNS, NNPS), and number (CD) benefited the most from the context, followed by adjective (JJ) and verb (VB, VBZ, VBG, VBN, VBD, VBP). Other tokens such as preposition (IN), coordinating conjunction (CC), etc. are less helped by context. We believe those that benefited less from the context are usually the ones that can be easily predicted from local context. 

Second, whether the target token appeared in the context or input has a large impact on the improvements. The input are the tokens preceding the target, corresponding to $x$ in Figure~\ref{fig:chunking}, and the context is $c^+$. Comparing the cases where target token is in context against the cases it's not, we can tell that the model is indeed utilizing information from the context and the presence of target token in context, regardless of whether it has already appeared in input, can help with the model prediction. If we compare the \texttt{In context, not in input} case with \texttt{In context, in input}, we can see that if the target token has already appeared in input, the benefit of appearing in context will be reduced, and if we compare \texttt{In context, in input} with \texttt{Not in context, in input}, we can see that target token in context is still beneficial even if it has already appeared in the input. Overall, this could be an evidence that the language models trained with our paradigm might copy from visible tokens when predicting the target token.

\begin{figure*}
\begin{center}
\includegraphics[width=1 \textwidth]{graphs/in_long_in_short.pdf}
\end{center}
\caption{Percentage of improvement on target log likelihood when there's context. We show the most frequent 20 POS tags, excluding punctuation. For the data on all the POS tags, see Appendix \todo{Add the table to appendix}.}\label{fig:in_long_in_short}
\end{figure*}

\subsection{Context Utility}

Following the observations in \ref{sec:long-short} we propose a metrics to estimate how much improvement a given context can give to the target. Using the same notation as before, let $\textbf{c}$ be the context tokens, $\textbf{x}$ be the input tokens and $\textbf{y}$ be the target tokens. The expected improvement on $\textbf{y}$ given $\textbf{x}$ and $\textbf{c}$ is then defined as:

\begin{equation}
\begin{split}
CU(\textbf{y}; \textbf{x}, \textbf{c}) = &\sum_{i}\mathbbm{1}(y_i \notin \textbf{c})\mathbbm{1}(y_i \notin \textbf{x})L_1(y_i) + \sum_{i}\mathbbm{1}(y_i \notin \textbf{c})\mathbbm{1}(y_i \in \textbf{x})L_2(y_i) + \\
&\sum_{i}\mathbbm{1}(y_i \in \textbf{c})\mathbbm{1}(y_i \notin \textbf{x})L_3(y_i) + \sum_{i}\mathbbm{1}(y_i \in \textbf{c})\mathbbm{1}(y_i \in \textbf{x})L_4(y_i)
\end{split}
\end{equation}

$L_1$ to $L_4$ are the expected improvement given the token's appearance in context and input. Specifically, $L_1$ is the expected improvement when the target token is not in context and not in input; $L_2$ is not in context, in input; $L_3$ is in context, not in input and $L_4$ is in context, in input. We estimate $L_i$ using a subset of C4 train split on a pre-trained decoder only language model. For each article, we vary the preceding token length as a way to emulate the presence or absence of context. Then we compute the average difference in log likelihood for each of the four conditions.

\subsubsection{Context Utility and Model Training}

When training the mT5 model for the language modeling experiment in Section~\ref{sec:lm-experiment}, we noticed an interesting phenomenon where the model with context will initially have the same behavior as the model without context, for a few hundred thousand steps. Then the training and validation accuracy will suddenly jump, as if the model "realized" the existence of context. From there on, the model with context will show a consistent lead over the one without context, to the end of training. This is depicted in Figure~\ref{fig:jump_warmstart}. One challenge with this jump is that there are a lot of variance on when it will happen. One way to address this is by first "warm start" the model with $100,000$ steps of training on a subset of training data with high Context Utility, then proceed on the full dataset. However, "warm start" does not improve the final model quality. It only makes training more reliable.

\begin{figure*}
\begin{center}
\includegraphics[width=0.6 \textwidth]{graphs/jump_warmstart.pdf}
\end{center}
\caption{Accuracy jump when training the language model from scratch.}\label{fig:jump_warmstart}
\end{figure*}

\subsection{Grounded Generation}

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c||cccc|c|}
\hline
\multirow{2}{*}{Original passages} & \multicolumn{4}{c|}{Output in passages}                                                                                                                         & Output not in passages \\ \cline{2-6} 
                                   & \multicolumn{4}{c|}{3354}                                                                                                                                       & 256                    \\ \hline \hline
\multirow{2}{*}{Filtered passages} & \multicolumn{1}{c|}{\shortstack{Output changed and \\ are still in passages}} & \multicolumn{1}{c|}{\shortstack{Output changed and are \\ no longer in passages}} & \multicolumn{1}{c|}{Output unchanged} & Excluded & -                      \\ \cline{2-6} 
                                   & \multicolumn{1}{c|}{2765}                          & \multicolumn{1}{c|}{261}                                & \multicolumn{1}{c|}{291}              & 37       & -                      \\ \hline
\end{tabular}%
}
\caption{Breakdown of the model output on Natural Question test split by whether.} \label{tab:nq_analysis}
\end{table}

In Natural Question task, we observed the model tends to copy from retrieved passages. To demonstrate this, we analyzed model output on the test split. For the following analysis we used the 1.56B model trained in~\ref{sec:natural_question}, and string matching is done with SQuAD~\cite{rajpurkar2016squad} normalization. To understand to what extend the model's outputs are from retrieved passages, we counted the number of examples whose outputs have appeared in any of the retrieval neighbors. Out of all 3610 outputs for the test split, 3354 (93\%) can be found in at least one of the top 20 DPR retrieved passages, and 1707 of them are correct answers. Furthermore, to quantify how many of those are due to memorization that happens to collide with the passages, we filtered out all the passages that contain model's output, and ran inference with the same model. With the colliding passages removed, 2765 outputs have appeared in the remaining retrieved passages. To see how the change in retrieval neighbors affects the model outputs, we compared the 3354 potentially copied outputs, before and after filtering. We found 2765 of them are changed, and the new outputs are still in the passages; 261 of them are changed to something no longer in the passages; 291 remain the same and 37 are excluded due to having less than 20 neighbors post filtering. For the 256 examples whose outputs are not previously in the passages, they are still not in the passages after filtering. The result is summarized in Table~\ref{tab:nq_analysis}. The 2765 outputs that are changed due to filtering are likely produced with the copying behavior. The rest are likely a combination of generalization and memorization that requires further investigation.

This analysis shed some light on the grounding behavior of the Encoder Decoder transformer model trained with QA tasks. There are still many unknowns such as under what condition the model will prefer copy over memorization. Nevertheless, it's still enlightening to see a model of moderate size with simple architecture can exhibit such behavior.

